Efficient Deterministic Quantitative Group Testing for Precise Information Retrieval

The Quantitative Group Testing (QGT) is about learning a (hidden) subset $K$ of some large domain $N$ using a sequence of queries, where a result of a query provides information about the size of the intersection of the query with the unknown subset $K$. Almost all previous work focused on randomized algorithms minimizing the number of queries; however, in case of large domains $N$, randomization may result in a significant deviation from the expected precision. Others assumed unlimited computational power (existential results) or adaptiveness of queries. In this work we propose efficient non-adaptive deterministic QGT algorithms for constructing queries and deconstructing a hidden set $K$ from the results of the queries, without using randomization, adaptiveness or unlimited computational power. The efficiency is three-fold. First, in terms of almost-optimal number of queries - we improve it by factor nearly $|K|$ comparing to previous constructive results. Second, our algorithms construct the queries and reconstruct set $K$ in polynomial time. Third, they work for any hidden set $K$, as well as multi-sets, and even if the results of the queries are capped at $\sqrt{|K|}$. We also analyze how often elements occur in queries and its impact to parallelization and fault-tolerance of the query system.

==> full-feedback-lower.tex <==
% !TEX root = main_constructive.tex
%
\section{Lower bound}
\label{sec:lower}
%\subsection{Full feedback}

%\begin{theorem}
%\label{thm:fulllower}
%If $n > k^2\log n/\log k$, then any solution to \gt under any $(\alpha,\beta)$-feedback has query complexity $\Omega\left(\frac{k^2}{\alpha^2 \log k}\right)$.
%\end{theorem}

\begin{theorem}
\label{lem:fulllower}
If $n > k^2\log n/\log k$, then any solution to \gt under any $(\alpha,\beta)$-feedback has query complexity 
$\Omega\left(\frac{k^2}{\alpha^2} \log^{-1} k\right)$.
\end{theorem}

\begin{proof}
%\textbf{of Theorem~\ref{thm:fulllower}}
An $(n,k,k)$-selector is a sequence of queries $Q_1,Q_2,\dots,Q_t$ such that for any $|K| \leq k$ and any element $x \in K$, for some query $Q$ we have $Q\cap K = \{x\}$. An $(n,k,k)$-selector is known to have query complexity $\Omega(\min\{n, (k^2/\log k) \cdot \log n\})$~\cite{ClementiMS01} and 
%a $(n,k,k)$-selector 
is known to exist with query complexity $O(k^2 \log n)$~\cite{erdos1985families}. Assume that $n$ is sufficiently large and let $c_1$ be such a constant that $(n,k,k)$-selector of query complexity $t_1 \leq c_1 (k^2/\log k) \cdot \log n $ does not exist; $c_1$ is well-defined by~\cite{ClementiMS01}. Let $c_2$ be a constant such that $(n,\alpha+1,\alpha+1)$-selector of size $t_2 \leq c_2 \alpha^2 \log n$ exists;
$c_2$ is well-defined by~\cite{erdos1985families}. Let $\mathcal{R}= \langle R_1, R_2, \dots, R_{t_2}\rangle$ be such a selector.

The proof of the theorem is by contradiction. Assume that there exists a sequence $\mathcal{Q} = \langle Q_1,Q_2,\dots, Q_t\rangle$ solving Group Testing with some $(\alpha,\beta)$-feedback function, such that the length of the sequence is $t \leq \frac{c_1}{c_2}\cdot \frac{k^2}{\alpha^2} \log^{-1} k$.

First we show the following fact: for any set $K \subset N$ of size $|K|\leq k$ and any element $x \in K$ there exists a set $Q$ in sequence $\mathcal{Q}$ such that $|K\cap Q| \leq \alpha + 1$. Assume the contrary and fix $K$ and $x$ that violate the fact. Observe that sets $K$ and $K\setminus \{x\}$ may produce the same feedback for any $(\alpha,\beta)$-feedback function (regardless of the value of $\beta$). This is because for any $Q_i$ such that $x\in Q_i$ we have $|Q_i \cap K| \geq \alpha + 2$ and $|Q_i \cap (K\setminus \{x\})| \geq \alpha + 1$. Hence, in the case of $Q_i \cap K$ the adversary may provide to the feedback function the same $\alpha$ elements as in $Q_i \cap (K\setminus \{x\})$. Since the feedback function is deterministic, the results will be the same, which is a contradiction with the fact that $\mathcal{Q}$ solves the Group Testing problem.

Next we transform $\mathcal{Q}$ into an $(n,k,k)$-selector: we take the $(n,\alpha+1,\alpha+1)$-selector $\mathcal{R}= \langle R_1, R_2, \dots, R_{t_2}\rangle$ and construct a sequence 
%
$\mathcal{S} = \langle Q \cap R \text{, for each } R = R_1, R_2, \dots, R_{t_2}   \text{, for each } Q = Q_1, Q_2, \dots, Q_t \rangle$.
The obtained family $\mathcal{C}$ has $t \cdot t_2 \leq t_1$ queries. We prove that it is also an $(n,k,k)$-selector.
%
For any set $K$ with $|K| \leq k$ and any $s \in S$ there exists, by the property of the sequence $\mathcal{Q}$ proved above, a set $Q$ in sequence $\mathcal{Q}$ such that $|Q \cap K| \leq \alpha + 1$. Now, since $\mathcal{R}$ is an $(n,\alpha+1,\alpha+1)$-selector, there exists a set $R$ in $\mathcal{R}$ such that $R\cap (Q \cap K) = \{x\}$. By the construction of $\mathcal{S}$, set $Q\cap R$ belongs to sequence $\mathcal{S}$, hence element $x$ is selected by family $\mathcal{S}$. Hence $\mathcal{S}$ is an $(n,k,k)$-selector. We know however that $(n,k,k)$-selector of length at most $t_1$ does not exist, and thus obtain a contraction showing that such a family $\mathcal{Q}$ cannot exist.
\end{proof}
%
Note that the lower bound formula $\Omega(\frac{k^2}{\alpha^2} \log^{-1} k)$ is equivalent to $\Omega(\frac{k^2}{\alpha\bar{\alpha}} \frac{\log(n/k)}{\log k})$, which bounds from below the query complexity of maximum expressiveness feedback.

==> lower-bound-size.tex <==

\subsection{Lower bound}

\begin{theorem}
Feedback $F$ does not admit $k \log^c n$ queries, for some constant $c$, for $\alpha=O(k^{\epsilon})$,
for sufficiently small $\epsilon$.
\end{theorem}

\begin{proof}
Może coś jak w sekcji 4 w pracy ktora wrzucilem: threshold... do katalogu papers?
\end{proof}

We consider an arbitrary fixed algorithm  defined by a sequence of queries $Q_1, Q_2, \ldots, Q_m$, and
a uniform distribution over $[n]_d$ for the
%two
input sets. 

We first estimate the probability for a fixed query $Q$ in $Q_1, Q_2, \ldots, Q_m$  that the size of the intersection o a
random set $X \in [n]_d$ with $Q$ is within the feedback interval.

\begin{lemma}\label{lemma:prob}
	Let $X$ be a random set uniformly chosen in $[n]_d$. For any fixed query
	$Q$, the probability that $|X \cap Q|$ falls within the feedback interval
	is $O(1/\log d)$.
\end{lemma}

\begin{proof}
	Let $q=|Q|$, 
	%$\mu = \frac{d}{2}$, $\delta = \frac{2}{\sqrt{d\log n}}$,
	%$x=\frac{d}{2} - {\frac{\sqrt{d}}{\log d}}$ and 
	%$y=\frac{d}{2} + {\frac{\sqrt{d}}{\log d}}$.
	the probability stated in the 
	%Lemma 
	lemma
	can be evaluated as follows.
	\begin{equation*}
	\prob \left( x \le |Q\cap X| \le y \right) 
	 = \sum_{i=x}^y \frac{\binom{q}{i}\cdot\binom{n-q}{d-i}}{\binom{n}{d}}.	
	\end{equation*}

We first prove the following upper bound:
\begin{equation}\label{eq:prob_v}
	\sum_{i=x}^y \binom{q}{i}\cdot\binom{n-q}{d-i}
	= O\left((y-x+1)\cdot
	\binom{n/2}{d/2}^2\right),
\end{equation}
and then we will show that the latter bound is actually $O(1/\log d)$.
	
To prove (\ref{eq:prob_v}) we can assume, without loss of generality,
that $q \ge n/2$ (the case $q \le n/2$ is symmetric). 
This proof is splitted in two cases depending on the value of $q$.

\medskip
\noindent
\textit{Case 1}: $n/2 \le q \le n/2 + n/(\sqrt{d}\log n)$. 	

\noindent
We have
\begin{eqnarray} 
\sum_{i=x}^{y} \binom{q}{i}\binom{n-q}{d-i}
&=& \sum_{i=x}^{d/2} \binom{q}{i}\binom{n-q}{d-i} 
+ \sum_{i=d/2+1}^{y} \binom{q}{i}\binom{n-q}{d-i} \nonumber\\
%&=& 
&\le &
\sum_{i=x}^{d/2} \binom{q}{d/2}\binom{n-q}{d/2} 
+ \sum_{i=d/2+1}^{y} \binom{q}{i}\binom{n-q}{d-i}, \label{key1}
\end{eqnarray}
where the last inequality holds because, for $i\le d/2$ and $q \ge n-q$:
\begin{equation}\label{e:aux:bin:eq:upper}
   \binom{q}{i}\binom{n-q}{d-i} \le \binom{q}{d/2}\binom{n-q}{d/2}.
\end{equation}
In order to prove (\ref{e:aux:bin:eq:upper}), it is sufficient to show that
\[
\binom{q}{i+1} \binom{n-q}{d-i-1}\ge  \binom{q}{i} \binom{n-q}{d-i}
\]
for $i<d/2$ and $q\ge n/2$. For brevity, we also assume that $d$ is even which combined
with $i<d/2$ implies that $i+1\le d/2$. Given these assumptions, we have
\begin{eqnarray} 
\binom{q}{i+1} \binom{n-q}{d-i-1}
&=& \binom{q}{i}\binom{n-q}{d-i} \cdot \frac{d-i}{i+1}\cdot \frac{q-i}{(n-q)-(d-i-1)} \\
&\ge & \binom{q}{i}\binom{n-q}{d-i} 
\end{eqnarray}
where the inequality follows from the facts that $\frac{d-i}{i+1}\ge 1$ because of $d-i>d/2$ and $i+1\le d/2$, while
$\frac{q-i}{(n-q)-(d-i-1)}\ge 1$ since $q-i\ge n/2-d/2$ while $(n-q)-(d-i-1)\le n/2-d/2$. This concludes the proof of (\ref{e:aux:bin:eq:upper}).

 
For $i > d/2$ and $q \le n/2 + n/(\sqrt{d} \log n)$, we have:
\begin{eqnarray*}
	\lefteqn{\binom{q}{i}\binom{n-q}{d-i}}\\ 
	&=&\binom{q}{d/2}\binom{n-q}{d/2} \cdot
    \frac{(d/2)!\ (d/2)!}{i!\ (d-i)!}\cdot
    \frac{(q-d/2)!\ (n-q-d/2)!}{(q-i)!\ (n-q-d+i)!}\\
	&=& \binom{q}{d/2}\binom{n-q}{d/2} \cdot 
	\frac{(d-i+1)\cdots(d/2)}{(d/2+1)\cdots(i)} \cdot
	\frac{(q-i+1) \cdots (q-d/2)}{(n-q-d/2+1)\cdots (n-q-d+i)}\\
%	&\le& \binom{q}{d/2}\binom{n-q}{d/2} \cdot
%	\frac{(q-d/2+1)\cdots(q-d/2)}{(n-q-d/2+1)\cdots (n-q-d/2)} \\
	&\le& 		
	\binom{q}{d/2}\binom{n-q}{d/2} \cdot
	\frac{\left(\frac{n}{2}+\frac{n}{\sqrt{d}\log n}-\frac{d}{2}\right)^{i-d/2}}{\left(\frac{n}{2}-\frac{n}{\sqrt{d}\log n}-\frac{d}{2}\right)^{i-d/2}}\\
	&\le& \binom{q}{d/2}\binom{n-q}{d/2} \cdot 
	\left( 1 + \frac{\frac{2n}{\sqrt{d}\log n}}{\frac{n}{2}-\frac{n}{\sqrt{d}\log n}-\frac{d}{2}} \right)^{\sqrt{d}/\log d }\\
	&=& \binom{q}{d/2}\binom{n-q}{d/2} \cdot 
	\left( 1 + \frac{2n}{\sqrt{d}\log n \left(\frac{n}{2}-\frac{n}{\sqrt{d}\log n}-\frac{d}{2}
	\right)} \right)^{\sqrt{d}/\log d }\\
    &\le &\binom{q}{d/2}\binom{n-q}{d/2} \cdot
    \left( 1 + \frac{4}{\sqrt{d}\log n -2}
    	\right)^{\sqrt{d}/\log d }\\
    &< & 4 \cdot \binom{q}{d/2}\binom{n-q}{d/2},
\end{eqnarray*}
where the second last inequality follows for $n$ sufficiently large and the 
last one for $d \ge 4$.
As an auxiliary inequality, we also show that
\begin{equation}\label{e:aux:bin:eq:lower}
\binom{q}{d/2}\binom{n-q}{d/2}\le \binom{n/2}{d/2}^2,
\end{equation}
provided that $q \ge n/2$. 
We consider $q > n/2$, as for $q = n/2$ the inequality is obvious.
For brevity we also restrict to the case that $n$ is even and therefore $n-q+1\le n/2$.
We derive (\ref{e:aux:bin:eq:lower}) from the following inequality
\[
\binom{q}{d/2}\binom{n-q}{d/2}\le \binom{q-1}{d/2}\binom{n-q+1}{d/2}
\]
satisfied for $q>n/2$. In order to prove this last inequality, we observe that
\begin{eqnarray*}
	\binom{q}{d/2}\binom{n-q}{d/2} &=& \binom{q-1}{d/2}\binom{n-q+1}{d/2}\cdot \frac{q}{n-q+1}\cdot \frac{(n-q+1)-d/2}{q-d/2}\\
	&\le& \binom{q-1}{d/2}\binom{n-q+1}{d/2}\cdot \frac{q}{n-q+1}\cdot \frac{(n-q+1)}{q}\\
	& = & \binom{q-1}{d/2}\binom{n-q+1}{d/2},
\end{eqnarray*}
%since $q\ge n-q+1$ 
where the inequality follows from the assumption $q\ge n-q+1$.

 
Resuming from (\ref{key1}) it follows that
\begin{eqnarray*}
  \sum_{i=x}^{y} \binom{q}{i}\binom{n-q}{d-i} 
      &\le& \sum_{i=x}^{d/2} \binom{q}{d/2}\binom{n-q}{d/2} +
            4\cdot\sum_{i=d/2+1}^{y} \binom{q}{d/2}\binom{n-q}{d/2} \\
      &\le& 4\cdot\sum_{i=x}^{y} \binom{q}{d/2}\binom{n-q}{d/2}   \\
      &\le& 4\cdot\sum_{i=x}^{y} \binom{n/2}{d/2}^2 \le 4\ (y-x+1)\cdot
      \binom{n/2}{d/2}^2,
\end{eqnarray*}
which concludes the proof of (\ref{eq:prob_v}) for $n/2 \le q \le n/2 + n/(\sqrt{d}\log n)$, i.e., in Case~1.

\medskip
\noindent
\textit{Case 2: $n/2 + n/(\sqrt{d}\log n) < q \le n$}.

\noindent
In order to prove (\ref{eq:prob_v}) in this case, 
we will first prove the following inequality:
\begin{equation}\label{eq:lb-sym-q}
\sum_{i=x}^y \binom{q}{i}\cdot\binom{n-q}{d-i}
\le
\sum_{i=x}^y \binom{n/2}{i}\cdot\binom{n/2}{d-i}
\end{equation}
	For $q \ge n/2$, we have 
\[
\sum_{i=x}^y \binom{q+1}{i} \binom{n-(q+1)}{d-i} = 
\sum_{i=x}^y \binom{q}{i} \binom{n-q}{d-i} \cdot\frac{(q+1)(n-q-d+i)}{(q-i+1)(n-q)}.
\]
Hence, to prove (\ref{eq:lb-sym-q}) it will be enough to show that
\[
     \frac{(q+1)(n-q-d+i)}{(q-i+1)(n-q)} \le 1.
\]


	We have,
	\[
	q \ge \frac{n}{2} + \frac{n}{\sqrt{d}\log d} 
      \ge (n+1)\left( \frac{1}{2} + \frac{1}{\sqrt{d}\log d} \right) - 1. 
	\]	
	From which we get
	\[
    qd \ge (n+1)\left( \frac{d}{2} + \frac{\sqrt{d}}{\log d} \right) - d 
       \ge (n+1)\cdot i - d. 
    \]
	where the last inequality follows from $i \le y =  \frac{d}{2}+\frac{\sqrt{d}}{\log d}$.
	This implies 
	\[
	-qd -d + i \le -in
	\] 
	and therefore, adding $nq - q^2 + iq +n -q$	to both sides, we obtain
	\[
	nq - q^2 - qd + iq +n -q -d +i \le nq -in +n -q^2 +iq -q.
	\]
	Hence,
	\[
	{(q+1)(n-q-d+i)} \le {(q-i+1)(n-q)},
	\]
	which concludes the proof of (\ref{eq:lb-sym-q}).
	

	
	
	We have that, for any $i< d/2$:
	\[
	\binom{n/2}{i}
	=
	\binom{n/2}{d/2} \cdot 
	\frac{(i+1)\cdot\ldots\cdot (d/2)}{((n/2)-(d/2)+1)\cdot\ldots\cdot ((n/2)-i)}
	\]
	and
	\[
	\binom{n/2}{d-i}
	=
	\binom{n/2}{d/2} \cdot 
	\frac{((n/2)-d+i+1)\cdot\ldots\cdot ((n/2)-(d/2))}{((d/2)+1)\cdot\ldots\cdot (d-i)}
	\]
	hence
	\[
	\binom{n/2}{i} \cdot \binom{n/2}{d-i}
	=
	\binom{n/2}{d/2}^2 \cdot 
	\frac{(i+1)\cdot\ldots\cdot (d/2)}{((n/2)-(d/2)+1)\cdot\ldots\cdot ((n/2)-i)}
	\]
	\[
	\cdot
	\cdot 
	\frac{((n/2)-d+i+1)\cdot\ldots\cdot ((n/2)-(d/2))}{((d/2)+1)\cdot\ldots\cdot (d-i)}
	\]
	\[
	=
	\binom{n/2}{d/2}^2 \cdot 
	\Pi_{j=1}^{d/2-i} \frac{i+j}{(n/2)-(d/2)+j} \cdot \frac{(n/2)-d+i+j}{(d/2)+j}
	\]
	\begin{equation}
	\label{eq:smaller}
	\le
	\binom{n/2}{d/2}^2 
	\ .
	\end{equation}
    To prove the last inequality, let us consider first the
    	case $i\le d/2$. 
	For every $i\le d/2$ and every 
	$1\le j\le d/2-i$,
	the difference between the denominator and the nominator of 
	\[
	\frac{i+j}{(n/2)-(d/2)+j} \cdot \frac{(n/2)-d+i+j}{(d/2)+j}
	\]
	in the product is
%\begin{eqnarray*}
%	&\phantom{.}&	
%	    \frac{n}{2}\cdot\frac{d}{2} - \frac{d^2}{4} -
%	    \left( i\cdot\frac{n}{2} -id +i^2 +2ij -jd\right)\\
%    &=&
%	    \frac{n}{2}\left( \frac{d}{2} - i\right)
%	    + i (d-i) +j (d-2i) -\frac{d^2}{4} \\
%	&\ge&
%    	\frac{n}{2}\left( \frac{d}{2} - i\right)
%	    + i (d-i) + (d-2i) -\frac{d^2}{4}\\
%	&\ge&     
%	0,
%\end{eqnarray*}
\begin{align*}
	\frac{n}{2}\cdot\frac{d}{2} - \frac{d^2}{4} -
	&\left( i\cdot\frac{n}{2} -id +i^2 +2ij -jd\right)\\
	&=
	\frac{n}{2}\left( \frac{d}{2} - i\right)
	+ i (d-i) +j (d-2i) -\frac{d^2}{4} \\
	&\ge
	\frac{n}{2}\left( \frac{d}{2} - i\right)
	+ i (d-i) + (d-2i) -\frac{d^2}{4}\\
	&\ge     
	%    	\frac{n}{2} 
	%        + \frac{d^2}{4} - \frac{d^2}{4} =	\frac{n}{2},
	0,
\end{align*}
where we have used the assumption
$j \ge 1$ in the second last inequality, the assumption that $i \le d/2$ and the given expression is a monotonically decreasing
function of $i$ in the last inequality.
 
%	\[
%	(n/2) \cdot ((d/2)-i) + (i+j)(d-i-2j) -d^2/4
%	\ ,
%	\]
%	which is a decreasing function in $j$ for all $j\ge 0$,
%	provided $d<3i$, which holds for sufficiently large $d$ as 
%	$i\ge x = \frac{d}{2} - \frac{\sqrt{d}}{\log n}$.
%	Therefore, this function is at least the value for $j=d/2-j$, which is
%	\[
%	(n/2) \cdot ((d/2)-i) + (d/2)i -d^2/4
%	\ ,
%	\]
%	for all the considered values of $j$.
%	This value is however always positive for $i<d/2$, because 
%	as a function of $i$ it is decreasing for all positive $i$,
%	provided $d\le n/2$, and its value for $i=d/2$ is $0$. 
%	%$nd/4 - d^4/4>0$.
	It follows that each factor in the product is smaller than or equal to $1$,
	which completes the proof of (\ref{eq:smaller}) for $i\le d/2$.
	
	The proof of (\ref{eq:smaller})
	for $i>d/2$ is by a symmetry argument, as
	\[
	\binom{n/2}{i} \cdot \binom{n/2}{d-i}
	\]
	for $i>d/2$ is equal to
	\[
	\binom{n/2}{j} \cdot \binom{n/2}{d-i}
	\]
	for $j=d-i<d/2$, and the latter was proved to be smaller than
	\[
	\binom{n/2}{d/2}^2
	\ .
	\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
%	\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
	
	Therefore, we have proved that for $n/2 + n/(\sqrt{d}\log n) < q \le n$:
	\[
	\binom{n/2}{i} \cdot \binom{n/2}{d-i} < \binom{n/2}{d/2}^2,
	\]
	which completes the proof of (\ref{eq:prob_v}) also in this case, i.e., in Case~2.

\medskip
	Now we use again Stirling's approximation (see (\ref{stirling})):
\[
\binom{n/2}{d/2}^2 <
\frac{2\pi (n/2)}{2\pi (d/2) \cdot 2\pi (n-d)/2} \cdot
\frac{(n/2)^{n}}{(d/2)^d (n-d)^{n-d}/2^{n-d}} \cdot
e^{1/(3n)-2/(6d+1)-2/(6n-6d+1)}
\]
\[
\le
c\cdot
\frac{n}{\pi d(n-d)} \cdot
\frac{n^{n}}{d^d (n-d)^{n-d}} 
\]
for some constant $c\ge e$.
Similarly,
\[
\binom{n}{d}
\ge
\sqrt{\frac{2\pi n}{2\pi d \cdot 2\pi (n-d)}} \cdot
\frac{n^{n}}{d^d (n-d)^{n-d}} \cdot
e^{1/(12n+1)-1/(12d)-1/(12n-12d)}
\]
\[
\ge
c'\cdot
\sqrt{\frac{n}{2\pi d(n-d)}} \cdot
\frac{n^{n}}{d^d (n-d)^{n-d}} 
\]
for some constant $c'\le 1/e$.
Hence, assuming that $d\le a \cdot n$ for any constant $a<1$, we get
\begin{equation*}
\frac{\binom{n/2}{d/2}^2}{\binom{n}{d}}
\le
(c/c')\sqrt{\frac{2}{\pi(1-a)}} \cdot \frac{1}{\sqrt{d}}
\ .
\end{equation*}

  Finally, recalling (\ref{eq:prob_v}), we can estimate the probability stated in the lemma:
 \begin{eqnarray*}
 	\prob \left( x \le |Q\cap X| \le y \right) 
 	&=&   \sum_{i=x}^y \frac{\binom{q}{i}\cdot\binom{n-q}{d-i}}{\binom{n}{d}}\\
 	&=& O\left( (y-x+1)
 	\frac{\binom{n/2}{d/2}^2}{\binom{n}{d}}\right)\\
 	&=&O\left(
 	\left(2{\frac{\sqrt{d}}{\log d}}+1\right) \cdot
 	(c/c')\sqrt{\frac{2}{\pi(1-a)}} \cdot \frac{1}{\sqrt{d}}\right)\\
	&=&
	O(1/\log d)
	\ .
	\end{eqnarray*}
	
\end{proof}

%Analogous reasoning could be done for any threshold interval $(x,y)$
%of length $2\sqrt{\frac{d}{\log n}}+1$, with $\mu=\frac{x+y}{2}$ 
%replacing $d/2$. 

Now, let us consider an arbitrary algorithm represented by any set of 
$m$ queries $Q_1,\ldots,Q_m$.
Assume that, the algorithm being correct, 
the sequence $Q_1,\ldots,Q_m$ separates each pair $X,Y\in [n]_d$.
For the sake of analysis, we introduce the notion of a \emph{bad query} with respect to a set $X$, \textit{i.e.}, a query whose intersection with $X$ has size in the feedback interval.
\begin{definition}[Bad query]
	A query set $Q\subseteq [n]$ is \textit{bad} with respect to a set $X\in [n]_d$
	when $|Q \cap X|$ falls within the feedback interval. 
\end{definition}
%
As a consequence of Lemma~\ref{lemma:prob}, there exists a constant $c>0$ such that, 
the expected number of bad queries for a random set 
$X\in [n]_d$ is at most $cm/\log d$. 

Let $\mathcal{X}$ be the family of those sets $X \in [n]_d$ for which the actual number of bad queries is at most $2cm/\log d$, i.e., it is at most twice as large as its expectation $cm/\log d$ for the uniform distribution of $[n]_d$.
Therefore, by Markov's inequality, the probability that a random set $X\in[n]_d$ does not belong to $\mathcal{X}$ is smaller than $1/2$. 
As our estimations are performed for the uniform distribution over the set $[n]_d$  of size ${n\choose d}$,
the size of $\mathcal{X}$ is at least $\frac12{n\choose d}$.
%By Markov's inequality and the fact that our estimations are done for the uniform distribution over $[n]_d$ (having size ${n\choose d}$)
%the size of $\mathcal{X}$ is at least $\frac12{n\choose d}$. 

%\begin{equation}
%\prob\left( |\mathcal{X}| \geq \frac{2c\cdot m}{\log n} \right) 
%\le \frac{\mathbf{E}\left[\sum_{i=1}^m Z_i\right] \cdot \log n}{2c\cdot m} = \frac{1}{2}.
%\end{equation}

According to the assumption that $Q_1,\ldots,Q_m$ separate each pair $X,Y\in [n]_d$,
there must be at least $\frac12{n\choose d}$ different feedbacks to be able to
distinguish all elements of $\mathcal{X}$.
On the other hand, the feedback for any set $X\in\mathcal{X}$ can be
encoded as follows. 
For each query $Q_i$, one bit encodes whether it is a bad query with respect to $X$. 
Then, if the query is bad, the intersection of $X$ and the query is inside the feedback interval.
And therefore the size of this intersection can be encoded in 
$$\log \left(2{\frac{\sqrt{d}}{\log d}}\right)$$ 
bits, where $2{\frac{\sqrt{d}}{\log d}}$ is the size of the feedback interval.
If the query is not bad on the other hand, we only receive information that the size of the intersection of $X$ and the query set is outside of the feedback interval and one bit is sufficient for encoding this fact.
Therefore, the size of the encoding of the whole feedback from $m$ queries is 
$$O\left(\log(d/\log d)\cdot \frac{2cm}{\log d}+2(m-\frac{2cm}{\log d})\right)=O(m),$$
since $c>0$ is constant and $d<n$. This in turn implies that the number of different feedbacks for
elements of $\mathcal{X}$ is $2^{O(m)}$. On the other hand, the size of $\mathcal{X}$ is
$$\Omega\left(\frac12{n\choose d}\right)=2^{\Omega\left({d\log(n/d)}\right)}.$$
This requires $m = \Omega (d \log(n/d))$ and the proof of~Theorem~\ref{???} is completed.




==> parity-feedback.tex <==
% !TEX root = main_constructive.tex
%
\section{Learning with restricted binary feedback}

\begin{theorem}
Lower bound $\Omega(\frac{k^2}{\alpha})$.
\end{theorem}

\begin{proof}

\end{proof}

\begin{theorem}
There is an explicit polynomial-time algorithm constructing non-adaptive queries and decoding the hidden set
from the feedback vector in polynomial time, for $O(\frac{k^2}{\alpha} \log^c n)$ queries, for some constant $c$.
\end{theorem}

\begin{proof}
Take the superimposed as above, but for $k/\alpha$ instead of $k$, and prove the following:
Each element occurs in an intersection of size at most $\alpha$.

Then replace each round with 1 by the selector of Lynch for $(n,\alpha)$, 0's by sequence of zeros of corresponding length.

This way we learn about all intersections of size at most $\alpha$, and from above property we know that
each node is in at least one such intersection.
Problem: what we learn from intersections of size bigger than $\alpha$? Would it be misleading for the desired learning from small intersections?
\end{proof}

